Stabilizing nanoparticles in the intensity minimum: feedback levitation on an inverted potential

We demonstrate the stable trapping of a levitated nanoparticle on top of an inverted potential using a combination of optical readout and electrostatic control. The feedback levitation on an inverted potential (FLIP) method stabilizes the particle at an intensity minimum. By using a Kalman-filter-based linear-quadratic-Gaussian (LQG) control method, we confine a particle to within $\sigma_x = (9.0 \pm 0.5) nm$ of the potential maximum at an effective temperature of $(16 \pm 1) K$ in a room-temperature environment. Despite drifts in the absolute position of the potential maximum, we can keep the nanoparticle at the apex by estimating the drift from the particle dynamics using the Kalman filter. Our approach may enable new levitation-based sensing schemes with enhanced bandwidth. It also paves the way for optical levitation at zero intensity of an optical potential, which alleviates decoherence effects due to material-dependent absorption and is hence relevant for macroscopic quantum experiments.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
